Global Collaboration through Local Interaction in Competitive Learning

Feature maps, that preserve the global topology of arbitrary datasets, can be formed by self-organizing competing agents. So far, it has been presumed that global interaction of agents is necessary for this process. We establish that this is not the case, and that global topology can be uncovered through strictly local interactions. Enforcing uniformity of map quality across all agents, results in an algorithm that is able to consistently uncover the global topology of diversely challenging datasets.The applicability and scalability of this approach is further tested on a large point cloud dataset, revealing a linear relation between map training time and size. The presented work not only reduces algorithmic complexity but also constitutes first step towards a distributed self organizing map.

==> Architecture.tex <==
The presented architectures  covers a power trading market besides, an underlying physical power network. 

As a power system is distributed in nature, HLA is used for exchange of information among distributed agents. It is a flexible architecture, hence, it is easier to customize to infrastructure requirements.

The main part of the a


\subsection{HLA - System of Systems}

High Level Architecture (HLA) is an IEEE standard for distributed simulation. Here, architecture is defined as: "\textit{Major functional elements, interfaces, and design rules, pertaining as feasible to all simulation applications, and providing a common framework within which specific system architectures can be defined}" \cite{HLA}. HLA is a standardized interaction architecture, which is used for exchange of information in distributed simulations. As described in \cite{HLA_DIS_7}, HLA has two main objectives, first is to have interoperability amongst heterogeneous simulations like real/non-real -time, event-driven, and live instrumented activities. And second objective is to reuse already developed simulations and their components.



Historically, HLA was designed for military purpose and it was used in a closed system but the usage of HLA is no more limited. In HLA, a federation is a composition of software modules knowns as federates. 


